On the benefits of index insurance in US agriculture: a large-scale analysis using satellite data

Index insurance has been promoted as a promising solution for reducing agricultural risk compared to traditional farm-based insurance. By linking payouts to a regional factor instead of individual loss, index insurance reduces monitoring costs, and alleviates the problems of moral hazard and adverse selection. Despite its theoretical appeal, demand for index insurance has remained low in many developing countries, triggering a debate on the causes of the low uptake. Surprisingly, there has been little discussion in this debate about the experience in the United States. The US is an unique case as both farm-based and index-based products have been available for more than two decades. Furthermore, the number of insurance zones is very large, allowing interesting comparisons over space. As in developing countries, the adoption of index insurance is rather low -- less than than 5\% of insured acreage. Does this mean that we should give up on index insurance? In this paper, we investigate the low take-up of index insurance in the US leveraging a field-level dataset for corn and soybean obtained from satellite predictions. While previous studies were based either on county aggregates or on relatively small farm-level dataset, our satellite-derived data gives us a very large number of fields (close to 1.8 million) comprised within a large number of index zones (600) observed over 20 years. To evaluate the suitability of index insurance, we run a large-scale simulation comparing the benefits of both insurance schemes using a new measure of farm-equivalent risk coverage of index insurance. We make two main contributions. First, we show that in our simulations, demand for index insurance is unexpectedly high, at about 30\% to 40\% of total demand. This result is robust to relaxing several assumptions of the model and to using prospect theory instead of expected utility.

==> Tables/SCYM_NASS_ave_corrs_rCrMsLo.tex <==
% latex table generated in R 4.1.1 by xtable 1.8-4 package
\begin{tabular}{lrrr}
  \toprule
Crop & Total ($\rho$) & By year ($\overline{\rho_t}$) & By county ($\overline{\rho_i}$) \\ 
  \midrule
Corn & 0.81 & 0.72 & 0.82 \\ 
  Soy & 0.77 & 0.70 & 0.75 \\ 
   \bottomrule
\end{tabular}


==> Tables/reg_EU_vs_none_Sstats_rEtIoWq.tex <==

\begin{table}
\caption{Utility of area versus no insurance: determinants at county level}
\begin{center}
\begin{tabular}{l c c c c c c c c}
\toprule
 & \multicolumn{4}{c}{Corn} & \multicolumn{4}{c}{Soy} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
 & (1) & (2) & (3) & (4) & (1) & (2) & (3) & (4) \\
\midrule
r2\_mean           & $0.33^{***}$ &              &             & $0.10^{***}$  & $0.11^{**}$ &              &              & $0.09^{***}$  \\
                   & $(0.04)$     &              &             & $(0.02)$      & $(0.04)$    &              &              & $(0.02)$      \\
temporal\_variance &              & $0.88^{***}$ &             & $0.95^{***}$  &             & $0.86^{***}$ &              & $1.09^{***}$  \\
                   &              & $(0.02)$     &             & $(0.02)$      &             & $(0.02)$     &              & $(0.03)$      \\
spatial\_variance  &              &              & $0.13^{**}$ & $-0.20^{***}$ &             &              & $0.44^{***}$ & $-0.30^{***}$ \\
                   &              &              & $(0.04)$    & $(0.02)$      &             &              & $(0.04)$     & $(0.03)$      \\
county\_mean       &              &              &             & $0.00$        &             &              &              & $0.00$        \\
                   &              &              &             & $(0.00)$      &             &              &              & $(0.00)$      \\
\midrule
R$^2$              & $0.11$       & $0.78$       & $0.02$      & $0.84$        & $0.01$      & $0.75$       & $0.19$       & $0.82$        \\
Num. obs.          & $597$        & $597$        & $597$       & $597$         & $597$       & $597$        & $597$        & $597$         \\
\bottomrule
\multicolumn{9}{l}{\scriptsize{Coefficients are standardized by re-scaling variables, hence no intercept is included.}}
\end{tabular}
\label{tab:reg-EU-vs-none-Sstats}
\end{center}
\end{table}

